Strategic Interactions between Large Language Models-based Agents in Beauty Contests

The growing adoption of large language models (LLMs) presents potential for deeper understanding of human behaviours within game theory frameworks. Addressing research gap on multi-player competitive games, this paper examines the strategic interactions among multiple types of LLM-based agents in a classical beauty contest game. LLM-based agents demonstrate varying depth of reasoning that fall within a range of level-0 to 1, which are lower than experimental results conducted with human subjects, but they do display similar convergence pattern towards Nash Equilibrium (NE) choice in repeated setting. Further, through variation in group composition of agent types, I found environment with lower strategic uncertainty enhances convergence for LLM-based agents, and having a mixed environment comprises of LLM-based agents of differing strategic levels accelerates convergence for all. Higher average payoffs for the more intelligent agents are usually observed, albeit at the expense of less intelligent agents. The results from game play with simulated agents not only convey insights on potential human behaviours under specified experimental set-ups, they also offer valuable understanding of strategic interactions among algorithms.

==> sections/learningreasoning.tex <==
\textbf{Reasoning.}
LLM-based agents were prompted at the beginning of period 1 to state their understanding of the game, and for each subsequent periods, they are asked to reinstate the goals.
This step is essential to mitigate the potential of them not comprehending the game.
Upon selecting a number, they were also asked to give a statement of reasoning in support of their choices.
From which, I found the low types appear to learn by either adjusting the reference point, and make selection that still comply with a strategic level of $0$, or via imitation through following the winner's past choice.
They may also not learn at all, and continue to select a number that they believe to be the popular choice.
As for the high types, they can learn by (1) anchoring their guesses to two-thirds of the past period's average; (2) imitating winner's strategy; (3) adjusting based on past period payoffs; and also (4) pattern recognition.
Agents may place different reliance on distinct pieces of historical information when making their choices, and multiple types of learning could come into play.
%The faster convergence to NE choice, which is indicative of stronger learning ability of the high type agents as compared to the low types, could be driven by the innate higher strategic level that carries throughout the periods, and also as a result of combined effect of learning from historical information.
